Coupling Global Context and Local Contents for Weakly-Supervised Semantic Segmentation

Thanks to the advantages of the friendly annotations and the satisfactory performance, Weakly-Supervised Semantic Segmentation (WSSS) approaches have been extensively studied. Recently, the single-stage WSSS was awakened to alleviate problems of the expensive computational costs and the complicated training procedures in multi-stage WSSS. However, results of such an immature model suffer from problems of background incompleteness and object incompleteness. We empirically find that they are caused by the insufficiency of the global object context and the lack of the local regional contents, respectively. Under these observations, we propose a single-stage WSSS model with only the image-level class label supervisions, termed as Weakly Supervised Feature Coupling Network (WS-FCN), which can capture the multi-scale context formed from the adjacent feature grids, and encode the fine-grained spatial information from the low-level features into the high-level ones. Specifically, a flexible context aggregation module is proposed to capture the global object context in different granular spaces. Besides, a semantically consistent feature fusion module is proposed in a bottom-up parameter-learnable fashion to aggregate the fine-grained local contents. Based on these two modules, WS-FCN lies in a self-supervised end-to-end training fashion. Extensive experimental results on the challenging PASCAL VOC 2012 and MS COCO 2014 demonstrate the effectiveness and efficiency of WS-FCN, which can achieve state-of-the-art results by 65.02\% and 64.22\% mIoU on PASCAL VOC 2012 val set and test set, 34.12\% mIoU on MS COCO 2014 val set, respectively. The code and weight have been released at:https://github.com/ChunyanWang1/ws-fcn.

==> sections/6_bib.tex <==
%-----------------------------------------------------------------------
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/wangchunyan.jpg}}]
{Chunyan Wang} is currently a Ph.D. student in School of Computer Science and Engineering, Nanjing University of Science and Technology, China. Before that, she received the BS degree and the MS degree in Computer Science and Technology at Nanjing Forestry University, China. Her research mainly focuses on deep learning, semantic segmentation and their applications. In these areas, she has published several journal papers including Neural Networks and Neurocomputing.
\end{IEEEbiography}
%-------------------------------------------------------------------------
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/zhangdong.jpg}}]{Dong Zhang} received his Ph.D. degree in computer science and technology from Nanjing University of Science and Technology in 2021. Dr. Zhang is now a postdoctoral research scientist at the Department of Computer Science and Engineering, The Hong Kong University of Science and Technology. His research interests include machine learning, image processing, computer vision and medical image analysis, especially in image classification, semantic image segmentation, object detection, and their potential applications. In these areas, he has published several journal and conference papers including IEEE Trans Cybern, PR, AAAI, ACM MM, IJCAI, ECCV, ICCV, CVPR, and NeurIPS.
\end{IEEEbiography}
%-------------------------------------------------------------------------
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/liyanzhang.jpg}}]
{Liyan Zhang} received the Ph.D. degree in computer science from the University of California, Irvine, Irvine, CA, USA, in 2014. She is currently a Professor with the College of Computer Science and Technology, Nanjing University of Aeronautics and Astronautics, Nanjing, China. Her research interests include multimedia analysis, computer vision, and deep learning. Dr. Zhang received the Best Paper Award from the International Conference on Multimedia Retrieval (ICMR) 2013 and the Best Student Paper Award from the International Conference on Multimedia Modeling (MMM) 2016.
\end{IEEEbiography}
%-------------------------------------------------------------------------
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/jinhuitang.jpg}}]
{Jinhui Tang} (Senior Member, IEEE) received the B.E. and Ph.D. degrees from the University of Science and Technology of China, Hefei, China, in 2003 and 2008, respectively. He is currently a Professor with the Nanjing University of Science and Technology, Nanjing, China. He has authored more than 150 articles in top-tier journals and conferences. His research interests include multimedia analysis and computer vision. Dr. Tang was a recipient of the Best Paper Awards in ACM MM 2007, PCM 2011, ICIMCS 2011, and ACM MM Asia 2020, the Best Paper Runner-Up in ACM MM 2015, and the Best Student Paper Awards in MMM 2016 and ICIMCS 2017. He has served as an Associate Editor for the IEEE TNNLS, the IEEE TKDE, and the IEEE TMM.
\end{IEEEbiography}
%-------------------------------------------------------------------------
